Robust Localized Multi-view Subspace Clustering

In multi-view clustering, different views may have different confidence levels when learning a consensus representation. Existing methods usually address this by assigning distinctive weights to different views. However, due to noisy nature of real-world applications, the confidence levels of samples in the same view may also vary. Thus considering a unified weight for a view may lead to suboptimal solutions. In this paper, we propose a novel localized multi-view subspace clustering model that considers the confidence levels of both views and samples. By assigning weight to each sample under each view properly, we can obtain a robust consensus representation via fusing the noiseless structures among views and samples. We further develop a regularizer on weight parameters based on the convex conjugacy theory, and samples weights are determined in an adaptive manner. An efficient iterative algorithm is developed with a convergence guarantee. Experimental results on four benchmarks demonstrate the correctness and effectiveness of the proposed model.

==> paper/table_regularizers.tex <==

\begin{table}
\small
\centering
\caption{ An example of regularizer $\psi(p)$ and its corresponding latent loss function $\phi(\ell)$ and minimizer function $\sigma(\ell)$, $\gamma$ is a hyper-parameter in $\{\phi(\ell), \psi(p), \sigma(\ell)\}$.}
%\setlength\tabcolsep{4.9pt}
\begin{tabular}{|c|c|c|}
%
\hline
\tabincell{c} {Latent function \\ $\phi(\ell)$}  & \tabincell{c} {Regularizer \\ $\psi(p)$ }
& \tabincell{c}  {Minimizer function \\ $\sigma(\ell)$}\\

\hline
$2(\sqrt{\gamma + \ell} - 1)$ & $\gamma p + 1/p - 2$ & $1/{\sqrt{\gamma + \ell}}$ \\

%\hline
%welsch & $\gamma (1 - \exp(-\frac{\ell}{\gamma}))$ & $\gamma p\ln p + \gamma(1-p)$ & $\exp(-\frac{\ell}{\gamma})$ \\

\hline
\end{tabular}
\label{examples_regularizers}
\end{table}

==> paper/table_vary_views.tex <==

\begin{table}[htp]
%	\small
	\centering
	\caption{Clustering Accuracy on USPS w.r.t. Number of Views.}
	\label{result_vary_views}
%	\setlength\tabcolsep{1pt}
	\begin{tabular}{|c|c|c|c|}
		\hline
		& SSC-AVG & SSC-WV & RMSC-SSC \\
		
		\hline
		2-views & & & \\
		
		\hline
		3-views & & & \\
		
		\hline
		4-views & & & \\
		
		\hline
		5-views & & & \\
		
		\hline
		6-views & & & 97.91 $\pm$ 0.03\\
				 
		\hline
	\end{tabular}	
\end{table}
